OntoEA: Ontology-guided Entity Alignment via Joint Knowledge Graph Embedding

Semantic embedding has been widely investigated for aligning knowledge graph (KG) entities. Current methods have explored and utilized the graph structure, the entity names and attributes, but ignore the ontology (or ontological schema) which contains critical meta information such as classes and their membership relationships with entities. In this paper, we propose an ontology-guided entity alignment method named OntoEA, where both KGs and their ontologies are jointly embedded, and the class hierarchy and the class disjointness are utilized to avoid false mappings. Extensive experiments on seven public and industrial benchmarks have demonstrated the state-of-the-art performance of OntoEA and the effectiveness of the ontologies.

==> tables/analyzeResults.tex <==
\begin{table}[ht]
\centering
\caption{The analysis of aligned entities generated by different models on the DW15kV1 dataset. 
\label{table:analyzeResult}}
\begin{tabular}{@{}lllll@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Ground Truth} & \multicolumn{2}{c}{Badcase} \\
      & Joint          & Conflict        & Joint        & Conflict     \\ \midrule
BoostEA      & 99.47\%        & 0.53\%          & 62.39\%      & 37.61\%      \\
MTransE      & -       & -         & -     & -     \\
\bottomrule
% \toprule
% \multirow{2}{*}{Model} & \multicolumn{2}{c}{Ground Truth} & \multicolumn{2}{c}{Badcase} \\
%       & Joint          & Conflict        & Joint        & Conflict     \\ \midrule
% BoostEA      & 99.47\%        & 0.53\%          & 62.39\%      & 37.61\%      \\
% MTransE      & -       & -         & -     & -     \\
% \bottomrule
\end{tabular}
\end{table}


==> tables/motivation.tex <==
\begin{table}[htb]
\centering
\caption{Misaligned entity pairs\label{table:motivation}}
\begin{tabular}{@{}ll@{}}
\toprule
\textbf{$e_1$ ($C_1$)} & \textbf{$e_2$ ($C_2$)}\\ 
\midrule
Bullet to Beijing (Film)        & Michael Caine (human)   \\
Duai National School (School)     & Gilberto Benetton (human)   \\
Charlie Major (MusicalArtist)             & To \& Fro (single)   \\ 
\bottomrule
% \textbf{E1 (entity in KG1)} & \textbf{E2 (entity in KG2)} & \textbf{Class of  E1} & \textbf{Class of  E2} \\ \midrule
% Bullet\_to\_Beijing         & Michael Caine               & Film                  & human                 \\
% Duai\_National\_School      & Gilberto Benetton           & School                & human                 \\
% Charlie\_Major              & To \& Fro                   & MusicalArtist         & single                \\ \bottomrule
\end{tabular}
\end{table}

